Diversity-aware $k$-median : Clustering with fair center representation

We introduce a novel problem for diversity-aware clustering. We assume that the potential cluster centers belong to a set of groups defined by protected attributes, such as ethnicity, gender, etc. We then ask to find a minimum-cost clustering of the data into $k$ clusters so that a specified minimum number of cluster centers are chosen from each group. We thus require that all groups are represented in the clustering solution as cluster centers, according to specified requirements. More precisely, we are given a set of clients $C$, a set of facilities $\pazocal{F}$, a collection $\mathcal{F}=\{F_1,\dots,F_t\}$ of facility groups $F_i \subseteq \pazocal{F}$, budget $k$, and a set of lower-bound thresholds $R=\{r_1,\dots,r_t\}$, one for each group in $\mathcal{F}$. The \emph{diversity-aware $k$-median problem} asks to find a set $S$ of $k$ facilities in $\pazocal{F}$ such that $|S \cap F_i| \geq r_i$, that is, at least $r_i$ centers in $S$ are from group $F_i$, and the $k$-median cost $\sum_{c \in C} \min_{s \in S} d(c,s)$ is minimized. We show that in the general case where the facility groups may overlap, the diversity-aware $k$-median problem is \np-hard, fixed-parameter intractable, and inapproximable to any multiplicative factor. On the other hand, when the facility groups are disjoint, approximation algorithms can be obtained by reduction to the \emph{matroid median} and \emph{red-blue median} problems. Experimentally, we evaluate our approximation methods for the tractable cases, and present a relaxation-based heuristic for the theoretically intractable case, which can provide high-quality and efficient solutions for real-world datasets.

==> algorithm.tex <==
\section{An exponential time approximation algorithm}

\cnote[Suhas]{Write the proof of the exponential time approximation algorithm.}

\subsection{Pruning the search space}
\cnote{Subset lattice pruning}


==> shrinking.tex <==
\subsection{Iterative distance shrinking}


\begin{algorithm}[t]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Facilities $F$ and group subsets $F_1,\ldots,F_t\subseteq F$, 
clients $C$, distance function $d:F\times C\rightarrow \reals$, 
total number of clusters $k$, group-level lower bounds $k_1,\ldots,k_t$.
}
\Output{Subset of facilities $S\subseteq F$ satisfying the diverse $k$-median problem instance.}

\ForEach{$((f,c)\in F\times C)$}{
	$d'(f,c) \leftarrow d(f,c)$\;
}
$i \leftarrow 0$\;
\While{$(i\text{\tt ++} < \text{\em max\_iter})$}{
	$S \leftarrow \kmedian(F,C,d',k)$\;
	\If{$(|S\cap F_j|\ge k_j$ \text{\em for all} $j\in[t])$} {
		return $S$\;
	}
	\ForEach{$(j\in[t])$}{
		$r_j \leftarrow \max\{k_j - |S\cap F_j|, 0\}$ \tcp*{deficit in facilities group $j$}
	}
	\ForEach{$(f\in F)$}{
		$J \leftarrow \{ j\in[t] \text{ s.t. } f\in F_j \}$ \tcp*{groups that facility $f$ belongs to}
		$R \leftarrow \{r_j \text{ s.t. } j\in J \text{ and } r_j>0\}$ \tcp*{set of non-zero deficities for facility $f$}
		$\sigma_f \leftarrow \discount(R)$ \tcp*{distance discount for facility $f$}
		\ForEach{$(c\in C)$}{
			$d'(f,c) \leftarrow \sigma_f\, d'(f,c)$\;
		}
	}
}
return $\emptyset$\;
\caption{\is($F,F_1,\ldots,F_t, C, d, k, k_1,\ldots,k_t$)}
\label{algorithm:iterative_shrinking}
\end{algorithm}


As another heuristic we first run the vanilla $k$-median problem without representation constraints. 
If the solution returned by the $k$-median algorithm does not satisfy 
the representation constraints for some groups, 
then we identify the facilities that belong to these groups
and we apply a discount function on the distances of these facilities to their clients.
The discounting process is repeated until we find a solution where all the representation constraints are satisfied, 
or when we reach a maximum number of iterations.
The proposed heuristic is illustrated in Algorithm~\ref{algorithm:iterative_shrinking}.

An important design choice is how to define the distance discount function. 
Two simple choices are the following:
\[
\discount(R) = 
\begin{cases} 
1-\epsilon & \text{if } R\ne\emptyset \\
1 & \text{otherwise}, \\
\end{cases} 
\text{ ~and~ }
\discount(R) = (1-\epsilon)^{|R|}.
\]
Notice that neither of these functions use the actual values $r_j$ in the set $R$, 
which express the amount by which the representation constraints are violated, 
instead both functions consider only the cardinality of the set $R$. 

\cnote[Aris]{
We may want to think of more elaborate discount functions, 
especially if these ones do not work well.
}




==> special-cases.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Special case without intersections}

%The inapproximability results described in Section~\ref{} hold only for the
%case with a non-empty intersection between the facility types. For the case
%with no interesecting facility types satisfying the constraints is trivial and hence
%our inapproximability results do not hold. Even though the problem is
%approximable it is \np-hard. In this section we will show that the problem
%variant without intersections can be reduced to an instance of the matroid median
%problem and hence a feasible algorithm for the matroid median problem can be
%used to solve the \divkmedian problem instances without intersecting facility types.


%\mpara{Diversified $k$-median problem without intersections.} The problem is an 
%instance of the \divkmedian problem such that  $F_i \cap F_j = \emptyset$ for all 
%$i \neq j$.

%Given a graph $G=(V,E)$, a collection $\mathcal{F}=\{F_1,\dots,F_t\}$ of subsets
%$F_i \subseteq V$ such that $F_i \cap F_j = \emptyset$ for all $i \neq j$, a
%constraint set $K = \{k_i \dots,k_t\}$ and an integet $k \leq n$. The problem
%asks us to find a subset $S \subseteq V$ such that $|S| = k$, $|F_i \cap S| \geq
%k_i$ for all $ i \in [t]$ and the cost function 
%$C(S) = \sum_{v \in V} \min_{s \in S} d(u,s)$ is minimised.

In this section we present a variant of the \divkmedian probem with only two
(red and blue) types of facilites and no intersections among the facility types.

\mpara{Diversified $rb$-median problem without intersections.}
Given a graph $G=(V,E)$, two set of facilities $F_1, F_2 \subseteq V$ such that
$F_1 \cap F_2 = \emptyset$, integers
$k_1, k_2 \leq n$.  The problem asks us to find a subset 
$S \subseteq \{F_1 \cup F_2\}$ such
that $|F_1 \cap S| \geq k_1$, $|F_2 \cap S| \geq k_2$ and the cost function
$C(S) = \sum_{v \in V} \min_{s \in S} d(u,s)$ is minimised. For simplicity, the
facilities $F_1$ and $F_2$ are refered as red and blue facilities, respectively.


The problem has a feasible solution if $\sum_{i \in [t]} k_i \leq k$. First we
present a local search algorithm for the case $k_1 + k_2 = k$. Later we show
that the general case with $k_1 + k_2 < k$ can be reduced to the former case
with only polynomially many feasible assignments for $k_1$ and $k_2$. Before
continuing with the algorithm let us introduce the \rbmedian problem.

\mpara{Red-blue median problem (\rbmedian).}
Given a graph $G=(V,E)$, two set of facilities $F_1, F_2 \subseteq V$, integers
$k_1, k_2 \leq n$.  The problem asks us to find a subset 
$S \subseteq \{F_1 \cup F_2\}$ 
such that $|F_1 \cap S| \leq k_1$, $|F_2 \cap S| \leq k_2$ and the cost function
$C(S) = \sum_{v \in V} \min_{s \in S} d(u,s)$ is minimised. For simplicity, the
facilities $F_1$ and $F_2$ are refered as red and blue facilities, respectively.

The \rbmedian problem accepts a $3 + \epsilon$ approximation algorithm based on
local-search~\cite{hajiaghayi2012local}.  The algorithm works by swapping a
red-blue pair $(r, b)$ with a red-blue pair $(r', b')$ until the cost is
improving, that is $C(S - r + r' - b + b') < C(S)$.  Note that $(r' = r, b' \neq
b)$, $(r' \neq r, b'=b)$ and $(r' \neq r, b' \neq b)$ are valid swap pairs.


==> supermodularity.tex <==
\begin{lemma}
The function $\sum_{i \in [t]} \frac{k_i}{|S \cap F_i| + 1}$ is supermodular.
\end{lemma}
\begin{proof}
We want to show $f(A\cap B) + f(A\cup B) \geq f(A) + f(B)$ for any $A,B \subseteq F$. Define $f_i(S)=\frac{k_i}{|S \cap F_i| + 1}$.

Take any $i$. We can consider without loss of generality that $A,B \subseteq F_i$. In addition, observe that
\begin{itemize}
\item adding 1 to the cardinality of an intersection or a union of sets is equivalent to adding a common element to both sets,
\item and the factor $k_i$ is common to all instances of $f_i$.
\end{itemize}
Thus, it is sufficient to analyze the function (abusing notation),
\[
f_i(A) = \frac{1}{|A|}.
\]

Now, 
\begin{align*}
f_i(A\cap B) + f_i(A\cup B)&= \frac{1}{|A\cap B|} + \frac{1}{|A\cup B|} = \frac{|A\cap B|+|A\cup B|}{|A\cap B||A\cup B|} = \frac{|A|+|B|}{|A\cap B||A\cup B|}
\\f_i(A) + f_i(B) &= \frac{|A|+|B|}{|A||B|}
\end{align*}
It will therefore be sufficient to show $|A\cap B||A\cup B| \leq |A||B|$.

Recall that $|A\cup B| = |A| + |B| - |A\cap B|$. Suppose $|A\cap B|=c$ and assume w.l.o.g. that $|A| \leq |B|$. Then,
\[
|A\cap B||A\cup B| = c(|A| + |B| - c).
\]
Clearly, $c\leq |A|$. If $c=|A|$, then $A\subseteq B$ and $|A\cap B||A\cup B|=|A||B|$. Otherwise, note that $c(|A| + |B| - c)$ increases in $c$, and thus any intersection smaller than $|A|$ results in $|A\cap B||A\cup B| < |A||B|$.
\end{proof}



==> tikz/local-search.tex <==
\begin{tikzpicture}[baseline=-1.25em,
    roundnode/.style={circle, draw=gray!60, fill=gray!20, very thick, minimum size=7mm},
  ]
  %Nodes
  \node[roundnode, diagonal fill={red!70}{blue!80}, minimum size=.5cm] at (0,2)  (a1)                                     {$f_1$};
  \node[roundnode, minimum size=.5cm, right = 2cm  of a1]   (a2) {};
  \node[roundnode, diagonal fill={red!70}{yellow!80}, minimum size=.5cm, right = 2cm of a2]  (a3)  {$f_3$};
  \node[roundnode, minimum size=.5cm, below = 2cm of a2]     (a4)  {};
  \node[roundnode, diagonal fill={green!70}{yellow!80}, minimum size=.5cm, left = 2cm of a4]     (a5)  {$f_2$};
  \node[roundnode, diagonal fill={green!80}{blue!80}, minimum size=.5cm, right = 2cm of a4]     (a6)  {$f_4$};

  \draw (a1) -- (a2) node[above, pos=0.5, black]{c};
  \draw (a1) -- (a4) node[above, pos=0.75, black]{c};
  \draw (a3) -- (a2) node[above, pos=0.5, black]{1};
  \draw (a3) -- (a4) node[above, pos=0.75, black]{1};
  \draw (a5) -- (a2) node[below, pos=0.75, black]{c};
  \draw (a5) -- (a4) node[below, pos=0.5, black]{c};
  \draw (a6) -- (a2) node[below, pos=0.75, black]{1};
  \draw (a6) -- (a4) node[below, pos=0.5, black]{1};
\end{tikzpicture}

